BANG: Billion-Scale Approximate Nearest Neighbor Search using a Single GPU

Approximate Nearest Neighbour Search (ANNS) is a subroutine in algorithms routinely employed in information retrieval, pattern recognition, data mining, image processing, and beyond. Recent works have established that graph-based ANNS algorithms are practically more efficient than the other methods proposed in the literature. The growing volume and dimensionality of data necessitates designing scalable techniques for ANNS. To this end, the prior art has explored parallelising graph-based ANNS on GPU, leveraging its massive parallelism. The current state-of-the-art GPU-based ANNS algorithms either (i) require both the dataset and the generated graph index to reside entirely in the GPU memory, or (ii) they partition the dataset into small independent shards, each of which can fit in GPU memory, and perform the search on these shards on the GPU. While the first approach fails to handle large datasets due to the limited memory available on the GPU, the latter delivers poor performance on large datasets due to high data traffic over the low-bandwidth PCIe interconnect. We introduce BANG, a first-of-its-kind technique for graph-based ANNS on GPU for billion-scale datasets, that cannot entirely fit in the GPU memory. BANG stands out by harnessing a compressed form of the dataset on a single GPU to perform distance computations while efficiently accessing the graph index kept on the host memory, enabling efficient ANNS on large graphs within the limited GPU memory. BANG incorporates highly optimised GPU kernels and proceeds in phases that run concurrently on the GPU and CPU, taking advantage of their architectural specificities. Using a single NVIDIA Ampere A100 GPU, BANG achieves throughputs 50x-400x higher than competing methods for a recall of 0.9 on three popular billion-scale datasets.

==> working_example.tex <==


%\subsection{An Illustrative Example}\label{ss:working_example}

% \begin{table*}
% \begin{tabular}{cccc}
%    \centering
%       \includegraphics[width=0.2\linewidth]{figures/toyExample.pdf} 
%       &
%       \scalebox{1}{
%       \begin{tabular}[t]{c|c|l|l}
%  & & Next & \\ 
% Iteration \# & Best\_L\_Set & Candidate & Neighbours \\ \hline
%  0 & \{6\} & 6 & \{8, 2\}\\ 
%  1 & \{8, 6, 2\} & 8 & \{6, 7\}\\
%  2 & \{8, 6, 7, 2\} & 7 & \{4, 8\}\\
%  3 & \{8, 6, 7, 2\} & 2 & \{0, 5\}\\
%  4 & \{8, 6, 7, 5\} & 5 & \{2, 9\}\\
%  5 & \{8, 9, 6, 7\} & 9 & \{5, 11\}\\
%  6 & \{8, 11, 9, 6\} & 11 & \{9, 10\}\\
%  7 & \{10, 8, 11, 9\} & 10 & \{8, 11\}
% \end{tabular}
% }
% &
%      \scalebox{1}{
%       \begin{tabular}[t]{c|c|l|l} 
%  & & Next & \\ 
% Iteration \# & Best\_L\_Set & Candidate & Neighbours \\ \hline
%  0 & \{6\} & 6 & \{8, 2\}\\ 
%  1 & \{8, 6, 2\} & 8 & \{6, 7\}\\
%  2 & \{8, 6, 7, 2\} & 7 & \{4, 8\}\\
%  3 & \{8, 6, 7, 2\} & 2 & \{0, 5\}\\
%  4 & \{8, 6, 7, 5\} & 5 & \{2, 9\}\\
%  5 & \{8, 9, 6, 7\} & 9 & \{5, 11\}\\
%  6 & \{8, 11, 9, 6\} & 11 & \{9, 10\}\\
%  7 & \{10, 8, 11, 9\} & 10 & \{8, 11\}
% \end{tabular}
% }
% &
%  \includegraphics[width=0.2\linewidth]{figures/toyExample.pdf} 
%  \end{tabular}
%  \caption{Testing typesetting}
% \end{table*}



% \begin{figure*}[t]
% % \begin{subfigure}
% %  \includegraphics[height=2.5cm,width=2.5cm,keepaspectratio]{figures/toyExample.pdf}
%     %\caption{ Graph}
%     %\label{fig:Sample Graph}
%  %\end{subfigure}
%  %\begin{subfigure}
%   %\includegraphics[height=4.5cm,width=2cm,keepaspectratio]%{old_plots/ToyExample-Page-2.drawio.pdf}
%    % \caption{PQ Distance}
%    % \label{fig:PQDist}
%  %\end{subfigure}
% %\begin{subfigure}
%   \includegraphics[height=4.5cm,width=4.5cm,keepaspectratio]{figures/toyExample.pdf}
% %\end{subfigure}
% %\begin{subfigure}
%   \includegraphics[height=4.5cm,width=2cm,keepaspectratio]{old_plots/ToyExample-Page-2.drawio.png}
% %  \end{subfigure}
% %\begin{subfigure}
%   \includegraphics[height=4.5cm,width=4cm,keepaspectratio]{old_plots/ToyExample-Page-3.drawio.pdf}
% %  \end{subfigure}
% %\begin{subfigure}
%   \includegraphics[height=4.5cm,width=4cm,keepaspectratio]{old_plots/ToyExample-Page-4.drawio.png}
%  % \end{subfigure}

%   %\includegraphics[width=0.6\linewidth]{figures/toyExample.tikz}
%   %\includegraphics[width=0.6\linewidth]{old_plots/ToyExample.png}
%    %\caption{Workflow of \ours on an illustrative example.}
%    \caption{Example illustrating \ours workflow for ANN search on \vamana graph.
%    The star indicates the query point $q(82,53)$.
%    }
%    \label{fig:workflow}
%   \end{figure*}
 %\tikz[baseline=-0.5ex]{\node[black!50,fill=green!75,star,inner sep=0pt,minimum size=3.5mm,draw];}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*} %[t]
\subfloat[]{
\label{fig:workflow:a}
 \begin{minipage}[t]{0.3\textwidth}
\vspace{-\topskip} 
\includegraphics[height=\linewidth,width=\linewidth,keepaspectratio]{figures/toyExample.pdf}
 \end{minipage}}
 \hfill
 \subfloat[]{
 \label{fig:workflow:b}
  \begin{minipage}[t]{0.17\textwidth}
\vspace{-\topskip} 
\setlength{\tabcolsep}{2pt}
 \scalebox{0.85}{
  \begin{tabular}{r|r|r}
         %\multirow{2}{*}{Node} & Cluster & \multicolumn{1}{l}{PQ} \\ %\hline
         Node & Cluster & \multicolumn{1}{l}{PQ} \\
         ID & ID & \multicolumn{1}{l}{Distance} \\\hline
         0 &  6& 6273 \\
         1 &  9& 3893\\
         2 &  7& 3233\\
         3 &  8& 3433\\
         4 &  1& 3973\\
         5 &  11& 2113\\
         6 &  0& 1033\\
         7 &  2& 1853\\
         8 &  4& 433\\
         9 &  5& 673\\
        10 &  3& 73\\
        11 &  10& 593\\
     \end{tabular}
     }
 \end{minipage}} 
 \hfill
  \subfloat[]{
  \label{fig:workflow:c}
  \begin{minipage}[t]{0.27\textwidth}
\vspace{-\topskip} 
 \includegraphics[height=\linewidth,width=\linewidth,keepaspectratio]{figures/ToyExample-Page-3.drawio.pdf}
 \end{minipage}}
 \hfill
\subfloat[]{
\label{fig:workflow:d}
\vspace{3.75\topskip}
  \begin{minipage}[t]{0.2\textwidth}
\vspace{-\topskip} 
\scalebox{0.85}{
\setlength{\tabcolsep}{2pt}
  \begin{tabular}{c|r|r}
         \multicolumn{1}{c|}{\multirow{2}{*}{Iteration \#}} & \multicolumn{1}{c|}{\multirow{2}{*}{Candidate}} & \multicolumn{1}{l}{Exact} \\
         && \multicolumn{1}{l}{Distance}\\\hline
         0 &  6& 1033 \\
         1 &  8& 433\\
         2 &  7& 1853\\
         3 &  2& 3233\\
         4 &  5& 2133\\
         5 &  9& 673\\
         6 &  11& 593\\
         7 &  10& 73\\ 
     \end{tabular}
     }
 \end{minipage}}
  \caption{Example illustrating {\normalfont \ours} workflow for ANN search on \vamana graph.
   The star indicates the query point $q(82,53)$.
   }
   \label{fig:workflow}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
% \begin{tabular}{c|c|l|l} 
%  & & Next & \\ 
% Iteration \# & Best\_L\_Set & Candidate & Neighbours \\ \hline
%  0 & \{6\} & 6 & \{8, 2\}\\ 
%  1 & \{8, 6, 2\} & 8 & \{6, 7\}\\
%  2 & \{8, 6, 7, 2\} & 7 & \{4, 8\}\\
%  3 & \{8, 6, 7, 2\} & 2 & \{0, 5\}\\
%  4 & \{8, 6, 7, 5\} & 5 & \{2, 9\}\\
%  5 & \{8, 9, 6, 7\} & 9 & \{5, 11\}\\
%  6 & \{8, 11, 9, 6\} & 11 & \{9, 10\}\\
%  7 & \{10, 8, 11, 9\} & 10 & \{8, 11\}
% \end{tabular}

% \begin{tabular}{r cl} \hline
% Graph Constructions Parameters:	 &  &  \\ \hline
% No of Nodes:  & 12 &  \\ 
% Dimensions:  & 2 &  \\ 
% Max Degree (out): & 2 &  \\ 
% No of Chunks:  & 1 &  \\ 
% \end{tabular}
% \bigskip

% \begin{tabular}{r cl} \hline
% Search Parameters: &  &  \\ \hline
% L\_search:   & 4 &  \\ 
% Recall parameter k:  & 2 &  \\ 
% Search Start: & Node 6(50,50)  &  \\ 
% %Query Point: & q (82,53)  &  \\ 
% Ground truth (2-Nearest neighbors): & 8,10  &   \\
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Search Results: &  &  \\ \hline
% Total Iterations: & 8 (0 - 7) & \\
% Our Algorithm returned ANNs:& 8 and 10 &  \\
% 2-recall@2: & 100\% & \\

% \end{tabular}
% \caption{Iterations in the working example}
% \label{table:example_iterations}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
% \begin{table}
% \begin{tabular}{r cl} \hline
% Iteration: & 0 &  \\ \hline
% Best\_L\_Set & 6 &  \\ 
% Next Candidate: & 6 &  \\ 
% Neighbours: & 8,2 &  \\ 
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Iteration: & 1 &  \\ \hline
% Best\_L\_Set & 8, 6, 2 &  \\ 
% Next Candidate: & 8 &  \\ 
% Children: & 6, 7 &  \\ 
% \end{tabular}

% \begin{tabular}{r cl} \hline
% Iteration: & 2 &  \\ \hline
% Best\_L\_Set & 8, 6, 7, 2 &  \\ 
% Next Candidate: & 7 &  \\ 
% Children: & 4, 8 &  \\ 
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Iteration: & 3 &  \\ \hline
% Best\_L\_Set & 8, 6, 7, 2 &  \\ 
% Next Candidate: & 2 &  \\ 
% Children: & 0, 5 &  \\ 
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Iteration: & 4 &  \\ \hline
% Best\_L\_Set & 8, 6, 7, 5 &  \\ 
% Next Candidate: & 5 &  \\ 
% Children: & 2, 9 &  \\ 
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Iteration: & 5 &  \\ \hline
% Best\_L\_Set & 8, 9, 6, 7 &  \\ 
% Next Candidate: & 9 &  \\ 
% Children: & 5, 11 &  \\ 
% \end{tabular}

% %\bigskip
% \begin{tabular}{r cl} \hline
% Iteration: & 6 &  \\ \hline
% Best\_L\_Set & 8, 11, 9, 6 &  \\ 
% Next Candidate: & 11 &  \\ 
% Children: & 9, 10 &  \\ 
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Iteration: & 7 &  \\ \hline
% Best\_L\_Set & 10, 8, 11, 9 &  \\ 
% Next Candidate: & 10 &  \\ 
% Neighbours: & 8, 11 &  \\ 
% \end{tabular}

% \begin{tabular}{r cl} \hline
% Graph Constructions Parameters:	 &  &  \\ \hline
% No of Nodes:  & 12 &  \\ 
% Dimensions:  & 2 &  \\ 
% Max Degree (out): & 2 &  \\ 
% No of Chunks:  & 1 &  \\ 
% \end{tabular}
% \bigskip

% \begin{tabular}{r cl} \hline
% Search Parameters: &  &  \\ \hline
% L\_search:   & 4 &  \\ 
% Recall parameter k:  & 2 &  \\ 
% Search Start: & Node 6(50,50)  &  \\ 
% Query Point: & q (82,53)  &  \\ 
% Ground truth (2-Nearest neighbors): & 8,10  &   \\
% \end{tabular}
% %\bigskip

% \begin{tabular}{r cl} \hline
% Search Results: &  &  \\ \hline
% Total Iterations: & 8 (0 - 7) & \\
% Our Algorithm returned ANNs:& 8 and 10 &  \\
% Recall@2: & 100\% & \\

% \end{tabular}
% \caption{Iterations in the working example}
% \label{table:example_iterations}
% \end{table}

% We demonstrate %our method 
%   %Figure~\ref{fig:workflow} depicts 
%   the workflow of \ours 
%   %technique 
%   through an illustrative example.  
%   %on an example input. 
 
\noindent\textbf{Distance Table Construction.}
Consider the toy example shown in Figure~\ref{fig:workflow}, having 12 points in the base dataset. The base dataset has two dimensions, and the data type of the coordinate values is an unsigned integer (1 byte, i.e., uint8).  
The compression technique involves representing a $d$-dimensional dataset vector with a compressed $m$-byte code, achieved by partitioning the $d$ dimensions into $m$ vector subspaces, %(or chunks), 
performing subspace clustering, and applying the quantization technique~\cite{PQ} for compression as outlined in Section~\ref{ss:pq}.
We specify m =1 for the product quantization. So, at the end of the compression step, each node (2 bytes long) will be represented by 1-byte. %as indicated below.

Before starting the search, we pre-compute the square of the Euclidean distances 
%(L2 distance) 
of all the cluster centroids 
%(pivots) 
to the query points on the GPU in parallel. 
Note that each subspace has $c$ clusters created using $k$-means clustering. 
This data structure is referred to as the PQ Distance table having dimensions $c \times m$ and it remains on GPU until the search terminates.
In the example, there are 12 clusters and one subspace, %(or chunk), 
so the dimensionality of the PQ Distance Table is $12 \times 1$. 
The distance between the query point and each cluster centroid is shown tabulated in Figure~\ref{fig:workflow:b}.
%beside the graph 
%in Figure~\ref{fig:workflow}.
%columns 1 and 3 of the \ref{table:pivot_table}. 
%Note: from an implementation optimization, we omit the final step of square root computation on the sum of squares of the diffs in each dimension.  
% After the PQ distance table is generated, we are ready to start the search. 
% The search begins from the medoid. We fetch all the neighbors of the medoid and look up the PQ clusters to which the respective nodes belong. 
% The distance of the respective cluster to the query point can be readily computed by summing the pre-computed distances from the PQ Distance table (referred to as distance computation using compressed vectors). We select the best L (closest neighbors) to the query point and end this iteration (iteration 0). 
After generating the PQ distance table, the search begins by retrieving neighbors of a node and determining the PQ clusters they belong to; the approximate distance to the query point is computed by summing pre-computed distances from the PQ Distance Table (compressed vectors).


% \begin{table}
% \begin{center}
% \begin{tabular}{|c| c |c |c|} 
%  \hline
%  \multicolumn{2}{|c|}{base dataset} &  \multicolumn{2}{|c|}{compressed  form}\\
%  \hline
%  base vector & Size (bytes) & compressed vector & Size (bytes) \\ [0.5ex] 
%  \hline\hline
%  [10,20] & 8 & [6] & 1 \\ 
%  \hline
%  [20,60] & 8 & [9] & 1 \\ 
%  \hline
%  [30,30] & 8 & [7] & 1 \\ 
%  \hline
%  [30,80] & 8 & [8] & 1 \\ 
%  \hline
%  [40,100] & 8 & [1] & 1 \\ 
%  \hline
%  [50,20] & 8 & [11] & 1 \\ 
%  \hline
%  [50,50] & 8 & [0] & 1 \\ 
%  \hline
%   [60,90] & 8 & [2] & 1 \\ 
%  \hline
%   [70,70] & 8 & [4] & 1 \\ 
%  \hline
%   [70,30] & 8 & [5] & 1 \\ 
%  \hline
%   [90,50] & 8 & [3] & 1 \\ 
%  \hline
%    [90,30] & 8 & [10] & 1 \\ 
%  \hline
% \end{tabular}
% \caption{Node ID to compressed vectors mapping }
% \label{table:compressed_vectors}
% \end{center}
% \end{table}

% The compression step does two things: (i) divide the d dimensions into m sub-spaces. In the above example, two dimensions are mapped on a single subspace. (ii) Within each subspace, the node is assigned to one out of n clusters. The max value for n is 255, as the cluster ID is represented by 1 byte. In the example, the quantizer created 12 clusters, and each node is mapped to 12 clusters. Each cluster will have a 2-dimensional centroid (aka pivot)) as shown in columns 1 and 2 of Table~\ref{table:pivot_table}:

% \begin{table}
% \begin{center}
% \begin{tabular}{|c| c | c|} 
%  \hline
%  Cluster ID & Centroid vector & PQ Dist\\ [0.5ex] 
%  \hline\hline
%  0 & [50, 50 ] & 1033 \\ 
%  \hline
%  1 & [40, 100] & 3973 \\ 
%  \hline
%  2 & [60, 90] & 1853 \\ 
%  \hline
%  3 & [80, 10] & 1853 \\ 
%  \hline
%  4 & [70, 70] & 433 \\ 
%  \hline
%  5 & [70, 70] & 673 \\ 
%  \hline
%  6 & [10, 20] & 6273 \\ 
%  \hline
%  7 & [30, 30] & 3233 \\ 
%  \hline
%  8 & [30, 80] & 3433 \\ 
%  \hline
%  9 & [20, 60] & 3893 \\ 
%  \hline
%  10 & [90, 50] & 73 \\ 
%  \hline
%  11 & [50, 20] & 2113 \\ 
%  \hline
% \end{tabular}
% \caption{Cluster ID to centroid mapping }
% \label{table:pivot_table}
% \end{center}
% \end{table}

% \begin{table}
% \begin{center}
% \begin{tabular}{|c| c | c|} 
%  \hline
%  Iteration \# & Candidate Node & Exact Dist\\ [0.5ex] 
%  \hline\hline
%  0 & 6 & 1033 \\ 
%  \hline
%  1 & 8 & 433 \\ 
%  \hline
%  2 & 7 & 1853 \\ 
%  \hline
%  3 & 2 & 3233 \\ 
%  \hline
%  4 & 5 & 2133 \\ 
%  \hline
%  5 & 9 & 673 \\ 
%  \hline
%  6 & 11 & 593 \\ 
%  \hline
%  7 & 10 & 73 \\ 
%  \hline

% \end{tabular}
% \caption{Re-ranking using exact distances between query point and best neighbor of every iteration }
% \label{table:re-ranking}
% \end{center}
% \end{table}


%\textbf{Graph Construction:} Here, we construct the adjacency list for each node using the \vamana technique. The \vamana is a directed graph, and we specify the max out degree as an input parameter to the graph construction activity. The resulting graph is shown in the above figure. The arrow direction indicates the node to its neighbor relationship.

% \textbf{CPU and GPU work distribution:} The bulk of the work occurs on the GPU during the search. The PQ Distance tables, neighbor filtering, and Distance computation of the nodes to query points using compressed vectors are performed on the GPU. The process of fetching the neighbors of a given node is the only step performed on the CPU. This step requires looking up the adjacency list in the graph data structure. Since the graph size runs into hundreds of GBs, it cannot be fitted in GPU. So, invariably it is stored on the RAM.

\noindent\textbf{ANN Search.}
%The ANN search is the GPU implementation of the modified Best First Search (BFS) over the graph index. 
%It is modified BFS in the sense that we use a bloom filter to filter out already considered neighbors and return the best candidate from the Parent set $P$ (not from BestL set $L$). 
%It entails
%performing 
%a breadth-first traversal %like traversal 
%on the index graph starting at a designated source vertex, the medoid. %(the medoid).
%

Each step(stage) annotated with the CUDA \textit{kernel} block in Figure~\ref{fig:arch} runs on an individual CUDA \textit{thread-block} (Section~\ref{ss:gpu_arch}) independently for each query. After all the queries execute a particular step, the execution proceeds to the next step. So, though the steps in the schema are sequential, within each step, queries can be handled in an embarrassingly parallel fashion.
% NOTE FROM KARTHIK : PLEASE RETAIN THE ESSENCE OF THE BELOW 4 SENTENCES (EVEN IF YOU DECIDE TO DELETE IT). BECAUSE, HOW WE ARE ACHIEVING PARALLELISM WITHIN THREADS OF A THREADBLOCK IS EASY FOR ANYONE TO UNDERSTAND (MULTITHREADING IS COMMON KNOWLEDGE). BUT HOW MULITPLE QUERIES ARE PARALLELISED USING THREADBLOCKS MAY NOT BE OBVIOUS TO SOME REVIEWERS. THE tEXT IN STEPS OF FIGURE INDICATE WHAT ACTIVITY IS DONE AT A QUERY OR THREADBLOCK LEVEL. THIS BACKGROUND WILL BE USED IN SEC 4.11 ALSO. 
% \textcolor{blue}{Note that each each query search executes in a separate CUDA \textit{ thread-block}. Each step shown shown under the CUDA Cores column, runs on a individual \textit{thread-block} in the figure in the context of the query. For each such step, there will be as many \textit{thread-blocks} as the number of queries.}
%We adopt the parallelization strategy of processing multiple queries in parallel. 
%This approach, in principle, promises an increased throughput, in terms of QPS, since lookup operations for all queries in a batch progress in tandem.
%Finally, a medoid in the base dataset is identified. 
Medoid will be used as the starting point for each query search. 
In the example shown in Figure~\ref{fig:workflow}, the medoid happens to be node 6.
Once the query is provided, the search starts from the medoid and iteratively progresses toward the query point. 
The worklist L is empty, so we initialize it with 6.
The entries in the worklist are always sorted in ascending order of their distance from the query point. 
We compute the distance of 6 from the query node using the PQ Distance table (i.e. compressed vectors).
With just one element in the worklist, node 6 is immediately selected as the \emph{candidate~node} for the next visit without the need for sorting.
We transfer node ID 6 from the GPU to the CPU and request the neighbours of node 6. 
The CPU-side implementation accesses the adjacency list to retrieve neighbours of node 6, providing the GPU with node IDs 8 and 2, concluding iteration 0.
%The CPU side implementation looks up the adjacency list and fetches the neighbours of 6 and returns node IDs 8 and 2 to GPU. This ends iteration 0.

In Iteration 1, GPU filters out previously visited nodes among the neighbours, computes their distances to the query point using the PQ Distance Table, sorts them, merges the sorted list with the worklist, and selects the first candidate node, which is node 8, to be visited next.
%For the next iteration, the neighbors of the first element (head) of Best L Set are fetched, and the distances re computed to the query point as explained previously. 
%Subsequently, we arrive at a new Best L set at the end of iteration 1. 
GPU maintains bloom filter data structure to keep track of visited nodes in order to avoid fetching neighbours of the same points and computing distances. 
%If a visited node is re-encountered, it will ignored for subsequent processing (i.e. neighbor filtering). 
In the figure, we can see that the set of neighbours progressively approaches the query point, and when all nodes in the worklist are visited, the iterations end.

% In the current example, iteration 0 starts with medoid, i.e.node 6. The Best L Set is empty so, we initialize it with 6. Best L set also maintains the distance of its elements from the query vector. 
% We compute the distance of 6 from the query node using the PQ Distance table (i.e. compressed vectors). Node 6 belongs to cluster 0 (from \ref{table:compressed_vectors}). The distance of cluster 0 to the query point can be computed from \ref{table:pivot_table} and is 1033 . Since there is only one element in the Best L set, there is no need for sorting it. We get straightaway pick node 6 as the candidate node to visit next. We transfer node id 6 to the CPU and request the neighbors of node 6. The CPU side implementation looks up the adjacency list and fetches the neighbours of 6 and returns node IDs 8 and 2 to GPU. This ends iteration 0.

% In Iteration 1, we filter the neighbors returned in the previous iteration to identify and exclude any already visited nodes. Nodes 8 and 2 are both un-visited. We compute the distance of each 8 from the query node using the PQ Distance table (i.e. compressed vectors). Node 8 belongs to cluster 4 (from \ref{table:compressed_vectors}). The distance of cluster 4 to the query point can be computed from \ref{table:pivot_table} and is 433 . Similarly, the distance of node 2 comes to 3233 . Now, the list of neighbors is sorted on the distances to the query vector, resulting a sorted list of neighbors: {8,2}. This list is merged with Best L Set using merge sort. The resulting Best L Set is: {8,6,2}. Note that Best L Set is always sorted and of fixed size. It represents the closest neighbors at the end of every iteration. The candidate node to visit will be the node at the head of Best L Set i.e. 8. Node ID 8 is sent to CPU implementation to fetch its neighbors. The GPU side receives the list of neighbors as: {6,7}. This ends in iteration 1.

% Similarly, iterations 2 -7 occur. Iterations end when there are no more un-visited nodes in the best L Set. So, at end of iteration 7 the best L set reads {10, 8, 11, 9}, and all are visited.

\noindent\textbf{Re-ranking.}
The candidate node identified and sent to CPU during each iteration is stored in a data structure for use in a final step called \emph{re-ranking}.
%The neighbours for each node visited during search are stored in a temporary data structure for use in a final search step called \emph{re-ranking}. 
A re-ranking process can compensate for inaccuracies in the search process caused by distance computation using compressed vectors~\cite{diskann}. 
Once the search process concludes, their exact distances from the query point are calculated on GPU using the exact base vectors, and the nodes are subsequently sorted based on these exact distances to extract the final k nearest neighbours from the list.
For the example, the sorted final list of candidate nodes, ordered by their distances to the query node, includes {10, 8, 11, 9, 6, 7, 5, 2}, resulting in the selection of the top 2 nearest neighbours, namely, 10 and 8.
Note that, for the re-ranking step, only full vectors of selected nodes are sent to GPU, which are fewer %less in number 
and can thus collectively fit into GPU memory for all queries.
%The best neighbor computed as part of each iteration is added to a list. We compute the distance of the nodes in this list to the query point using the exact base vectors. The nodes are sorted in ascending order based on distances computed. The final set of k nearest neighbors is extracted from this list. The re-ranking is performed on GPU.

% The list of candidate Nodes in each iteration is captured in \ref{table:re-ranking}. For each node, we compute the exact distance (i.e. L2 distance) with the query point. In Iteration 0, the candidate node (i.e. the node that was sent to CPU for neighbor fetching) is 6. Its exact distance is 1033 . Similarly, for the rest of the candidate nodes exact distance is calculated, as shown in the table. The sorted list of Candidate Nodes based on their distance to the query Node will be: {10, 8, 11, 9, 6, 7. 5, 2}. To return the final result of k-Nearest Neighbours (k=2), the first k-elements from this list are returned i.e. 10 and 8.


